Think Rationally about What You See: Continuous Rationale Extraction for Relation Extraction

Relation extraction (RE) aims to extract potential relations according to the context of two entities, thus, deriving rational contexts from sentences plays an important role. Previous works either focus on how to leverage the entity information (e.g., entity types, entity verbalization) to inference relations, but ignore context-focused content, or use counterfactual thinking to remove the model's bias of potential relations in entities, but the relation reasoning process will still be hindered by irrelevant content. Therefore, how to preserve relevant content and remove noisy segments from sentences is a crucial task. In addition, retained content needs to be fluent enough to maintain semantic coherence and interpretability. In this work, we propose a novel rationale extraction framework named RE2, which leverages two continuity and sparsity factors to obtain relevant and coherent rationales from sentences. To solve the problem that the gold rationales are not labeled, RE2 applies an optimizable binary mask to each token in the sentence, and adjust the rationales that need to be selected according to the relation label. Experiments on four datasets show that RE2 surpasses baselines.

==> subfiles/2_related.tex <==
% \input{tables/dataset}

\section{Related Work}
\label{related}

\subsection{Fact-Checking Datasets} 

Table~\ref{tab:dataset} summarized fact-checking dataset by grouping them into two types: real-world and synthetic \cite{guo2021}. 
% Existing datasets can be grouped into two types: real-world and synthetic ~\citep{guo2021}. 
Real-world dataset consists of claims that originates from the media ecosystem and are fact-checked by dedicated agencies (e.g. PolitiFact). Synthetic datasets contain claims created artificially by mutating sentences from Wiki articles. Early efforts predicted the veracity based solely on the claims or metadata \cite{Rashkin2017TruthOV, Wang2017LiarLP}, but studies show that predictions without considering evidence fail to identify misinformation \cite{Schuster2020TheLO}. Therefore, synthetic datasets \cite{Thorne18Fact,jiang2020hover,vitaminc2021} considered Wikipedia as the source of evidence and annotated the sentences from articles as evidence.  
% Although these datasets incorporated evidence, they restricted world knowledge to a single source (i.e. Wikipedia), ignoring the challenge of collecting evidence from heterogeneous sources. 
However, these efforts restricted world knowledge to a single source (i.e. Wikipedia), which is not ideal to develop systems that collect evidence from heterogeneous sources. On the other hand, real-world efforts~\cite{Hanselowski2019ARA, kotonya2020health} extracted summaries accompanying fact-checking articles about the claims as evidence. Nonetheless, using fact-checking articles is not realistic, as they are not available during inference. To address this issue, other datasets~\cite{Augenstein2019MultiFCAR, gupta-srikumar-2021-x} included search snippets generated by Google as evidence. Unlike prior real-world efforts, we propose to directly incorporate retrieved documents to provide more information for better verification.


\subsection{Fact-Checking Systems} 
When verifying synthetic claims, systems often operate as a pipeline consisting of an evidence extraction module and a verification module. Relevant articles are first retrieved from the Wikipedia dump by using entity linking, or TF-IDF~\citep{hanselowski-etal-2018-ukp,Thorne18Fact}.  After obtaining the evidence sentences, a textual entailment model is applied for verifying the claim~\citep{luken-etal-2018-qed, Nie2019CombiningFE}. Recent systems employ graph-based models to aggregate evidence. This allows the verification of more complex claims where several pieces of information can be combined~\citep{Zhou2019GEARGE, Liu2020KernelGA, Zhong2020ReasoningOS, schlichtkrull2020}. Due to the difficulty of annotating evidence under real-world scenarios, most systems assume the evidence sentences are given, ignoring the challenge of evidence extraction~\citep{Hanselowski2019ARA,Augenstein2019MultiFCAR,kotonya2020health,gupta-srikumar-2021-x}. Different from these methods, we propose to model the evidence extraction as a latent variable. Such a design enables our system to extract evidence from web sources and validate real-world claims based on evidence found on the Internet. 


% When verifying synthetic claims, systems often operate as a pipeline consisting of an evidence extraction module and a verification module~\citep{guo2021}, as the annotation of evidence sentences are provided. Relevant articles are first retrieved from the Wikipedia dump by using entity linking, or TF-IDF~\citep{hanselowski-etal-2018-ukp,Thorne18Fact}. Then a fine-grained module can be trained to extract related sentences from retrieved articles~\citep{nie-etal-2019-revealing, Nie2019CombiningFE,Liu2020KernelGA}. After obtaining the evidence sentences, a textual entailment model is applied for the claim verification~\citep{luken-etal-2018-qed, Nie2019CombiningFE}. Recent systems employ graph-based models to aggregate evidence. This allows the verification of more complex claims where several pieces of information can be combined~\citep{Zhou2019GEARGE, Liu2020KernelGA, Zhong2020ReasoningOS, schlichtkrull2020}. Due to the difficulty of annotating evidence under real-world scenarios, most systems assume the evidence sentences are given, ignoring the challenge of evidence extraction~\citep{Hanselowski2019ARA,Augenstein2019MultiFCAR,kotonya2020health,gupta-srikumar-2021-x}. Different from these methods, we propose to model the evidence extraction as a latent variable. Such a design enables our system to extract evidence from web-sources and validate real-world claims based on evidence found on the Internet. 

% Some early work does not include evidence retrieval at all, performing verification purely on the basis of surface forms and metadata~\citep{Wang2017LiarLP,Rashkin2017TruthOV,Dungs2018CanRS}. Recently \citet{lee-etal-2020-language} 
% considered using the information stored in the weights of a large pretrained language model -- BERT~\citep{Devlin2019BERTPO} -- as the only source of evidence, as it has been shown competitive in knowledge base completion \citep{petroni-etal-2019-language}.
% Without explicitly considering evidence such approaches are likely to propagate biases learned during training, and render justification production impossible~\citep{lee-etal-2021-towards,PanCXKW20}.


% Similarly, evidence can be re-ranked implicitly during verification in late-fusion systems
% %late-fusion strategies where evidence is re-ranked implicitly as part of the verification system have also been proposed
% ~\citep{ma-etal-2019-sentence, schlichtkrull2020}.


%The primary challenge for retrieval systems is scale -- the number of articles in potential information sources such as Wikipedia, LexisNexis, or Google News is massive. Retrieval modules are therefore very limited in how much processing can be spent on each potential piece of evidence. This challenge has been addressed through  various
% Recently, dense retrievers employing learned representations and fast dot-product indexing~\citep{johnson2017faiss} have shown strong performance~\citep{lewis2020retrieval, maillard-etal-2021-multi}. %Efficient retrieval often comes as the expense of precision. To alleviate this,

% An alternative approach was proposed by \citet{Fan2020GeneratingFC}, who retrieved evidence using question generation and question answering via search engine results. 
% Some work avoids retrieval by making a \textit{closed-domain assumption} and %, i.e.\ assuming access to an oracle retriever, and 
% evaluating in a setting where appropriate evidence has already been found~\citep{Ferreira2016EmergentAN,Chen2020TabFactAL, zhong-etal-2020-logicalfactchecker, yang-etal-2020-program, eisenschlos-etal-2020-understanding}; this, however, is unrealistic. Finally, \citet{allein2021time} took into account the timestamp of the evidence in order to improve veracity prediction accuracy.

% What to do with evidence


==> subfiles/8_limitation.tex <==
\section{Limitation}
\label{limitation}


In this paper,  we propose to incorporate full text of web pages returned by the search engine for verifying real-world claims. Though the proposed fact-checking system significantly outperforms the baselines, it still has the following three major limitations. Firstly, the training corpus only contains claims selected and verified by fact-checkers, as it is crawled from fact-checking agencies. Fact-checkers select and verify claims based on their judgements as well as public interests. Thus, there is no guarantee that the training corpus can cover any topics. Secondly, evidence in the retrieved web pages can be exhibited in the tables, PDFs, images, audios and videos. Human fact-checkers are able to extract relevant information from these heterogeneous sources, while our fact-checking system can only extract textual sentences as evidence. Unlike an artificial fact-checking dataset that assumes the world knowledge is restricted to Wikipedia, real-world dataset requires knowledge from more diversified sources. Using a search engine is an effective approach to obtain related knowledge, but it also brings the concern of untrustworthy evidence. Not all web documents returned by the search engine are equally trustworthy, and sometimes trustworthy sources contradict each other. Almost all existing fact-checking systems including ours are not able to address the presence of disagreeing or untrustworthy evidence. 

